Quantum Radio Astronomy: Quantum Linear Solvers for Redundant Baseline Calibration

The computational requirements of future large scale radio telescopes are expected to scale well beyond the capabilities of conventional digital resources. Current and planned telescopes are generally limited in their scientific potential by their ability to efficiently process the vast volumes of generated data. To mitigate this problem, we investigate the viability of emerging quantum computers for radio astronomy applications. In this a paper we demonstrate the potential use of variational quantum linear solvers in Noisy Intermediate Scale Quantum (NISQ) computers and combinatorial solvers in quantum annealers for a radio astronomy calibration pipeline. While we demonstrate that these approaches can lead to satisfying results when integrated in calibration pipelines, we show that current restrictions of quantum hardware limit their applicability and performance.

==> Makefile <==
TEX_SOURCES =	qradio.tex

BIB_SOURCES =	references.bib

FIG_SOURCES =	

JGR_SOURCES =	

JPG_SOURCES =	

PDF_SOURCES =	

PNG_SOURCES =	

STY_SOURCES =	

AUX_FILES =	$(TEX_SOURCES:%.tex=%.aux)
GEN_FIGURES =	$(FIG_SOURCES:%.fig=%.pdf) $(JGR_SOURCES:%.jgr=%.pdf)

FIGURES =	$(GEN_FIGURES) $(JPG_SOURCES) $(PNG_SOURCES) $(PDF_SOURCES)

GEN_EXT =	bbl blg dvi idx ilg ind lof log lot ps toc ps_pages
GEN_FILES =	$(AUX_FILES) $(GEN_FIGURES) qradio.pdf $(GEN_EXT:%=qradio.%)\
		mfput.log missfont.log texput.log

TEXINPUTS =	inputs:.:
TEXFONTS =	:

%.pdf:		%.jgr
		jgraph $< | epstopdf --filter > $@

%.pdf:		%.fig
		fig2dev -L pdf $< $@

qradio.pdf:	$(TEX_SOURCES) $(STY_SOURCES) $(BIB_SOURCES) $(FIGURES)
		TEXINPUTS=$(TEXINPUTS) TEXFONTS=$(TEXFONTS) pdflatex qradio
		bibtex qradio
		TEXINPUTS=$(TEXINPUTS) TEXFONTS=$(TEXFONTS) pdflatex qradio
		TEXINPUTS=$(TEXINPUTS) TEXFONTS=$(TEXFONTS) pdflatex qradio

qradio.ps:	qradio.pdf
#		pdftops -paper letter qradio.pdf
		pdftops -paper A4 qradio.pdf

evince::	qradio.pdf
		evince $<

okular::	qradio.pdf
		okular $<

xpdf::		qradio.pdf
		xpdf -g 900x1200 $<

lpr::		qradio.ps
		lpr $<

clean::
		rm -f $(GEN_FILES)

